SAINT: Spatially Aware Interpolation NeTwork for Medical Slice Synthesis

Deep learning-based single image super-resolution (SISR) methods face various challenges when applied to 3D medical volumetric data (i.e., CT and MR images) due to the high memory cost and anisotropic resolution, which adversely affect their performance. Furthermore, mainstream SISR methods are designed to work over specific upsampling factors, which makes them ineffective in clinical practice. In this paper, we introduce a Spatially Aware Interpolation NeTwork (SAINT) for medical slice synthesis to alleviate the memory constraint that volumetric data poses. Compared to other super-resolution methods, SAINT utilizes voxel spacing information to provide desirable levels of details, and allows for the upsampling factor to be determined on the fly. Our evaluations based on 853 CT scans from four datasets that contain liver, colon, hepatic vessels, and kidneys show that SAINT consistently outperforms other SISR methods in terms of medical slice synthesis quality, while using only a single model to deal with different upsampling factors.

==> backup.tex <==
 
% (A small paragraph for RFN. How to go from two-view SISR to the final interpolated CT)
% \subsection{3D CT to 2D Disentanglement}

% While our assumption is that between-slices images canbe well resolved by 2D kernels due to their similar distor-tion, the constrained 3D field of view means that the result-ing images in aggregate will create directional artifact oneach slice. Since every pixel has 8 numbers along 4 axes, weperform inference on each of these axis, and overlay themas channels for the fusion stage.  As such, for every voxel,there are 4 approximations of it based on all the availableaxes, and the fusion stage further determines the validity ofeach  approximation  by  considering  the  slice-wise  consis-tency.


 
 %, which includes a formulation that considers the changing voxel resolution of $I^{x}(y,z)$ and $I^{y}(x,z)$. 

% As $I^{x}_{\downarrow r_z}(y,z)$ and $I^{y}_{\downarrow r_z}(x,z)$ have anisotropic resolution between $z$ and $x, y$ axes, we propose a spatially aware upsampling formulation that incorporates the physical resolutions of the three axes, denoted as $R_x$, $R_y$, and $R_z$. %Fig. \ref{fig:MSR} demonstrates the pipeline of AMI.
% Using a meta-upsampling structure inspired by Meta-SR, we use the anisotropic images $I^{x}_{\downarrow k}(y,z)$ and $I^{y}_{\downarrow k}(x,z)$ to predict the missing voxels through the sub-pixel convolutional layer and the periodic shuffling operator proposed by []. 


%As each value on $F^{y}_{\downarrow r_z}(x,z)$ is a feature representation of $I^{y}_{\downarrow r_z}(x,z)$, 


%While Meta-SR enables non-integer upsampling rate, it achieves so by generating a set of filters for every HR pixel. In contrary, in our formulation, $W$ only consists of $r_z-1$ sets of filters. Therefore, for $F^{x}_{\downarrow k}(y,z) \in \mathbb{R}^{inC \times Y \times Z}$, we require $\frac{Y\times Z}{r_z-1}$ times less memory than Meta-SR for filter generation. While we do not innately support non-integer upsampling factor, Meta-SR only showed slightly better performance on large non-integer upsampling factors against the zoom-ins of over-upscaled image. 

%Furthermore, Meta-SR did not take into consideration the different underlying voxel spacing of every medical volume.  

% Consider $F^{x}_{\downarrow k}(y,z)$ as a tensor with shape $inC \times Y \times Z$, and the generated filters to have size $k$, Meta-SR needs to generate filters of size $inC \times 1 \times Y \times Z \times k^$


% There are several factors that make Meta-SR hard to be applied practically. Firstly, Meta-SR generates a set of filters for every HR pixel, which occupy massive amount of memory. Secondly, there exists no dataset that has nature pairs of HR images and their non-integer downscaled version. This leads to the model learning to reverse the interpolation, rather than estimating for the true underlying pixels. 

%Hu et al. \cite{Hu_2019_CVPR} proposed Meta-SR, which employs a 


%In order to achieve flexibility in upsampling factors, we employ a similar idea as the Meta-Upscale Module proposed by , where the convolutional filters $W(x,z,c)$ at the upsampling stage are dynamically generated. We propose a Kernel Distance Mapping (KDM) as the input to the Anisotrpoic Meta Interpolation stage, in order to incorporate the spatial resolution of the $x$, $y$, $z$ axes, of which we denote as $R_X$, $R_Y$, $R_Z$.







% A meta upsampling structure only needs to generate kernels of size $G*(r_x*r_y-1)*kernsize*kernsize$ in order to predict the missing voxels. Compare to Meta-SR's implementation, which generates kernels of size $G*W_out*H_out*kernsize*kernsize$, massive number of parameters are saved. While we sacrifice some flexibility for arbitrary upsampling factor, as described in related work, the downside can be ameliorated by over-upsampling and downsample with little effect on performance. 

% \subsubsection{Kernel Distance Mapping}
%  For each convolution operation, the convolutional filter takes a patch from the LR feature map and produces an approximation of the central pixel on the respective channel. Since we know the coordinate transform between the generated channels $T$ and the SR image $PS(T)$, for each voxel that the filter observes, we can calculate its relative physical distance with respect to the voxel that the filter produces. For filters of size $k$, we call such relationship a Kernel Distance Mapping $\mathcal{P} \in \mathbb{R}^{k\times k\times c}$, which can be calculated as the following:
%  \begin{align}
%  \begin{split}
%      &\mathcal{P}(x,y,c) = \\
%      &\norm{(\mathcal{M}(x,y,0)-\mathcal{M}(\floor*{\frac{k}{2}}, \floor*{\frac{k}{2}},c))\cdot(R_X, R_Y, R_Z)}_{2} \\
%      & x \in [0,k-1], y \in [0,k-1], c \in [1,r_z]
%  \end{split}
%  \end{align}

% KDM is unique for every channel $c$, and does not change by pixel coordinates. For every channel, KDM is calculated and provided to the Anisotropic Interpolation stage to generate respective filters of size $inC*r_z*k*k$. $F^{x}_{\downarrow r_z}(y,z)$ and $F^{y}_{\downarrow r_z}(x,z)$ is then convolved with the kernels, and the resulting channels are rearranged to form the SR image.

% Notice that instead of super-resolving 2D slices independently, we propose to take a slab of $s$ slices as input and estimate a single SR output. Using a larger $s$ allows more context to be modelled. AMI is repeated for all $x$ and $y$.
% Finally, the super-resolved slices can be reformatted as sagittally and coronally super-resolved volumes, $I_{sag}(x,y,z)$ and $I_{cor}(x,y,z)$, respectively. We apply the following $L_1$ loss to train the SISR network:
% \begin{align}
%     \mathcal{L}_{AMI} &= \lVert \mathcal{G}_{\theta}(\mathbb{I}^{x,s}_{\downarrow r_z}) - I^{x}_{gt} \rVert_1 + \lVert \mathcal{G}_{\theta}(\mathbb{I}^{y,s}_{\downarrow r_z}) - I^{y}_{gt} \rVert_1,
% \end{align}
% where $I^{x}_{gt} = I^x(y, z)$ and $I^{y}_{gt} = I^y(x, z)$ in the highly sampled volume.

% From the axial perspective, $I_{sag}(x,y,z)$ and $I_{cor}(x,y,z)$ provide line-by-line estimations for the missing axial slices. However, since no constraint is enforced on the estimated axial slices, the interpolations lead to directional artifacts (See Section \ref{sec:ablation_study}). Furthermore, since AMI only explores information from non-axial dimensions, a second, RFN stage is needed to recover the correlations on the axial dimension.


% \input{seg/seg_result.tex}
%In Fig. \ref{fig:Seg}, we demonstrate the advantage of the proposed method in brain matter segmentation. It is clear that although 2D and 3D CNN generates visually plausible interpolation as presented in Fig. \ref{fig:Comparison}, the brain matters are easily misclassified due to incorrect anatomical structures and blurred details.

% unique challenges: 1. 3D, 2. need to be flexible in many distortion level, as in a hospital they don't have a week to train a model and then view a upsampled version, 3. image quality need to be high, but not overly smooth or has possiblity to have fictitious details

% While CT and MR images are 3D by principle, the imaging is typically done through capturing consecutive 2D slices and merging. 

%-------------------------------------------------------------------------


==> figures/abaltion_rfn.tex <==
\begin{table}[h!]
\centering 
\small
\begin{tabular}{|l | c | c |c |}
\hline
 PSNR/SSIM & Liver & Colon & Hepatic Vessels \\
\hline
 $RFN^{2D}_{2 View}$  & 34.90/0.9602& 34.19/0.9579 & 34.47/0.9630  \\
\hline
 $RFN^{2D}_{4 View}$  & 34.97/0.9607&34.23/0.9582 &34.53/0.9633  \\
\hline
 $RFN^{3D}_{4 View}$  &34.97/0.9606&34.26/0.9583 &34.55/0.9634  \\
\hline
\end{tabular}
\caption{}
\label{table:se-net}
\end{table}

==> figures/ablation_backup.tex <==
\begin{table*}[t!]
\small
\centering 
\begin{tabular}{|l | c|c|cccc c |}
\hline
 PSNR(dB)/SSIM& Scale &Parameters&Liver & Colon & Hepatic Vessels & Lung & Kidney \\
% \hline
% \multirow{ 2}*{Bicubic}  & x4 &  &  &  &  &   \\
%  & x6 &  &  &  &  &  \\
\hline
\multirow{ 2}*{2D MDSR}  & x4 & \multirow{ 2}*{2.92M} & 33.43/0.9471 & 32.76/0.9436 & 32.91/0.9490 & 30.55/0.8733 & 34.57/0.9508 \\
 & x6 & & 31.15/0.9237 & 30.16/0.9133 & 30.22/0.9216 & 29.14/0.8486 & 32.30/0.9297 \\
\hline
\multirow{ 2}*{2D RDN} & x4 & \multirow{ 2}*{2.77M} &34.22/0.9546 & 33.39/0.9511 & 33.74/0.9571 & 31.15/0.8875 &35.17/0.9550  \\
 & x6 & & 31.78/0.9315 & 30.82/0.9232 & 31.13/0.9319 & 29.58/0.8603 & 32.47/0.9314 \\
\hline
\multirow{ 2}*{Meta-SR} & x4 &\multirow{ 2}*{2.81M} &34.2/0.9541 & 33.51/0.9516 & 33.74/0.9570 & 30.88/0.8814 & 35.08/0.9544 \\
 & x6 & &31.88/0.9322 & 30.86/0.9234 & 31.09/0.9318 & 29.35/0.8539 & 32.60/0.9329 \\
\hline
\multirow{ 2}*{AMI} & x4 & \multirow{ 2}*{2.79M}&34.40/0.9561 & 33.65/0.9529 & 33.93/0.9586 & 31.28/0.8918 & 35.28/0.9560 \\
 & x6 & & 32.05/0.9333&30.99/0.9249 &31.22/0.9333 & 29.74/0.8635 & 32.72/0.9343 \\
\hline
\end{tabular}
\vspace{-1pt}
\caption{Quantitative Comparison of AMI against alternative methods}
\label{exp:sota_table}
\vspace{-1pt}
\end{table*}

==> figures/ablation_visual.tex <==
\begin{figure*}[t!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}[b]{cccc}
        \begin{subfigure}[b]{0.25\linewidth}
            \includegraphics[width=\textwidth,height=0.75\textwidth]{visualization_imgs/ablation_img/hr_2.png}
            \caption{HR}
            \label{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.25\linewidth}
            \includegraphics[width=\textwidth,height=0.75\textwidth]{visualization_imgs/ablation_img/meta_2.png}
            \caption{Meta-SR}
        \end{subfigure} &
        \begin{subfigure}[b]{0.25\linewidth}
            \includegraphics[width=\textwidth,height=0.75\textwidth]{visualization_imgs/ablation_img/rdn_2.png}
            \caption{RDN}
        \end{subfigure} &
        \begin{subfigure}[b]{0.25\linewidth}
            \includegraphics[width=\textwidth,height=0.75\textwidth]{visualization_imgs/ablation_img/saint_2.png}
            \caption{AMI}
        \end{subfigure} 
    \end{tabular}
    \caption{}
\end{figure*}

==> figures/ablation_visual_v2.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{figure*}[t!]
\captionsetup[subfigure]{labelformat=empty}
\begin{tabularx}{\textwidth}{ |c| *{5}{Y}| }
\hline

Factor & MDSR & RDN & Meta-RDN & SAINT & HR\\
\hline
4 &
\begin{subfigure}[t]{0.18\textwidth}
    \centering
    \includegraphics[width=\linewidth,height=0.75\textwidth]{visualization_imgs/ablation_img/mdsr_x4.png}
\end{subfigure} &
\begin{subfigure}[t]{0.18\textwidth}
    \centering
    \includegraphics[width=\linewidth,height=0.75\textwidth]{visualization_imgs/ablation_img/msr_x4.png}
\end{subfigure} &
\begin{subfigure}[t]{0.18\textwidth}
    \centering
    \includegraphics[width=\linewidth,height=0.75\textwidth]{visualization_imgs/ablation_img/meta_x4.png}
\end{subfigure} &
\begin{subfigure}[t]{0.18\textwidth}
    \centering
    \includegraphics[width=\linewidth,height=0.75\textwidth]{visualization_imgs/ablation_img/saint_x4.png}
\end{subfigure} &
\begin{subfigure}[t]{0.18\textwidth}
    \centering
    \includegraphics[width=\linewidth,height=0.75\textwidth]{visualization_imgs/ablation_img/hr.png}
\end{subfigure}\\

\hline

\end{tabularx}
\vspace{-1em}
\caption{Visual comparisons of slice interpolation approaches. For 4x sparsity, the second of three interpolated MR slices is presented. For 8x sparsity, the third of seven interpolated slices is presented.}\label{fig:Comparison}
\end{figure*}




==> figures/different_noise.tex <==
\begin{figure}[t!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}[b]{cc}
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth,height=0.75\textwidth]{visualization_imgs/axial_noise.png}
            \caption{Axial Metal Artifact}
            \label{fig:intro_ma}
        \end{subfigure} &
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth,height=0.75\textwidth]{visualization_imgs/sagittal_noise.png}
            \caption{Sagittal Metal Artifact}
        \end{subfigure} \\
    \end{tabular}
    \caption{Metal Artifact, as shown in an axial and sagittal slice of the same volume. The red boxes on the bottom left show the magnified  effect of metal artifact away from the metal location.}
\end{figure}

==> figures/kernels.tex <==
\begin{figure}[t!]
  \centering
  \includegraphics[height=0.22\textheight,width=0.4\textwidth]{visualization_imgs/kernels.png}
  \caption{Comparison of (a) 3D kernel and (b) possible non-axial 2D kernels estimated through AMI.} %All light green boxes represent values of zeros}
\label{fig:stitching_artifact}
\end{figure}

==> figures/quantitative_backup.tex <==
\begin{table*}[t!]
\small
\centering 
\begin{tabular}{|l | c|c|cccc c |}
\hline
 PSNR(dB)/SSIM& Scale &Parameters&Liver & Colon & Hepatic Vessels & Lung & Kidney \\
\hline
\multirow{ 2}*{Bicubic}  & x4 && 28.36/0.8733&28.01/0.8622 & 27.83/0.8720 & 26.54/0.7862 & 30.33/0.8946   \\
 & x6 &&26.57/0.8405& 26.28/0.8265 & 26.00/0.8382 & 25.06/0.7348 & 28.59/0.8635  \\
\hline
\multirow{ 2}*{3D MDSR}  & x4 && 33.70/0.9487 & 32.79/0.9442 & 32.80/0.9480 & 31.57/0.8940 &  35.36/0.9563\\
 & x6 && 31.18/0.9237 & 29.99/0.9122 & 29.95/0.9192 & 29.91/0.8652 &  \\
\hline
\multirow{ 2}*{mDCSRN} & x4 &&  &  &  &  &  \\
 & x6 &&  &  &  &  &  \\
\hline
\multirow{ 2}*{3D RDN} & x4 && 33.88/0.9509 & 32.96/0.9467 & 32.99/0.9506 & 31.69/0.8956 & 35.43/0.9570 \\
 & x6 && 31.52/0.9286 & 30.54/0.9204 & 30.49/0.9263 & 30.01/0.8662 & 32.71/0.9339 \\
\hline
\multirow{ 2}*{SAINT} & x4 && 34.97/0.9607 & 34.23/0.9582 & 34.53/0.9633 & 31.65/0.8976 & 35.87/0.9601 \\
 & x6 &&  &  &  &  &  \\
\hline
\end{tabular}
\vspace{-1pt}
\caption{Quantitative evaluation of 3D SISR approaches in terms of PSNR and SSIM.}
\label{exp:sota_table}
\vspace{-1pt}
\end{table*}

==> figures/supplemental_img.tex <==
\begin{figure*}[!htb]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
        \begin{tabular}[b]{c c c c c c c}
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{1pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x4/ax/hr_big.png}
                \caption*{Ground Truth}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.07\linewidth}
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=2\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x4/ax/hr.png}
                \caption*{HR}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x4/ax/bicu.png}
                \caption*{Bicubic}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x4/ax/mdcsrn.png}
                \caption*{mDCSRN}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x4/ax/mdsr.png}
                \caption*{3D MDSR}
            \end{subfigure}
            &
            % \hspace{-21pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x4/ax/msr.png}
                \caption*{3D RDN}
            \end{subfigure}
            &
            % \hspace{-10pt}
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x4/ax/saint.png}
                \caption*{SAINT}
            \end{subfigure}\\
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{1pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x4/sag/hr_big.png}
                \caption*{Ground Truth}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.07\linewidth}
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=2\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x4/sag/hr.png}
                \caption*{HR}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x4/sag/bicu.png}
                \caption*{Bicubic}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x4/sag/mdcsrn.png}
                \caption*{mDCSRN}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x4/sag/mdsr.png}
                \caption*{3D MDSR}
            \end{subfigure}
            &
            % \hspace{-21pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x4/sag/msr.png}
                \caption*{3D RDN}
            \end{subfigure}
            &
            % \hspace{-10pt}
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x4/sag/saint.png}
                \caption*{SAINT}
            \end{subfigure}\\            
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{1pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x4/ax/hr_big.png}
                \caption*{Ground Truth}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.07\linewidth}
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=2\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x4/ax/hr.png}
                \caption*{HR}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x4/ax/bicu.png}
                \caption*{Bicubic}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x4/ax/mdcsrn.png}
                \caption*{mDCSRN}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x4/ax/mdsr.png}
                \caption*{3D MDSR}
            \end{subfigure}
            &
            % \hspace{-21pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x4/ax/msr.png}
                \caption*{3D RDN}
            \end{subfigure}
            &
            % \hspace{-10pt}
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x4/ax/saint.png}
                \caption*{SAINT}
            \end{subfigure}\\
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{1pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x4/sag/hr_big.png}
                \caption*{Ground Truth}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.07\linewidth}
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=2\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x4/sag/hr.png}
                \caption*{HR}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x4/sag/bicu.png}
                \caption*{Bicubic}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x4/sag/mdcsrn.png}
                \caption*{mDCSRN}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x4/sag/mdsr.png}
                \caption*{3D MDSR}
            \end{subfigure}
            &
            % \hspace{-21pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x4/sag/msr.png}
                \caption*{3D RDN}
            \end{subfigure}
            &
            % \hspace{-10pt}
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x4/sag/saint.png}
                \caption*{SAINT}
            \end{subfigure}\\        
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{1pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x4/ax/hr_big.png}
                \caption*{Ground Truth}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.07\linewidth}
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=2\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x4/ax/hr.png}
                \caption*{HR}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x4/ax/bicu.png}
                \caption*{Bicubic}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x4/ax/mdcsrn.png}
                \caption*{mDCSRN}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x4/ax/mdsr.png}
                \caption*{3D MDSR}
            \end{subfigure}
            &
            % \hspace{-21pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x4/ax/msr.png}
                \caption*{3D RDN}
            \end{subfigure}
            &
            % \hspace{-10pt}
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x4/ax/saint.png}
                \caption*{SAINT}
            \end{subfigure}\\
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{1pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x4/sag/hr_big.png}
                \caption*{Ground Truth}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.07\linewidth}
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=2\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x4/sag/hr.png}
                \caption*{HR}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x4/sag/bicu.png}
                \caption*{Bicubic}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x4/sag/mdcsrn.png}
                \caption*{mDCSRN}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x4/sag/mdsr.png}
                \caption*{3D MDSR}
            \end{subfigure}
            &
            % \hspace{-21pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x4/sag/msr.png}
                \caption*{3D RDN}
            \end{subfigure}
            &
            % \hspace{-10pt}
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x4/sag/saint.png}
                \caption*{SAINT}
            \end{subfigure}\\                    
        \end{tabular}
    \caption{Visual comparisons of different methods against SAINT for $r_z = 4$. The difference maps are provided to the right of the results for better visualization. %For mDCSRN, distortion due to stitching smaller 3D patches are visible, as indicated by the red arrows. 
    Images are best viewed when magnified.} \label{fig:supp_visual_x4}
    %(a) is an slice from the Kidney dataset. Despite lower PSNR value compare to RDN, SAINT generates much clearer details. (b) is a slice from the Hepatic Vessels dataset. Note that the mDCSRN result has some minor artifact due to stitching individually infered 3D cubes together
    \vspace{-1em}
\end{figure*}

==> figures/supplemental_img_x6.tex <==
\begin{figure*}[!htb]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
        \begin{tabular}[b]{c c c c c c c}
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{1pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x6/ax/hr_big.png}
                \caption*{Ground Truth}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.07\linewidth}
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=2\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x6/ax/hr.png}
                \caption*{HR}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x6/ax/bicu.png}
                \caption*{Bicubic}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x6/ax/mdcsrn.png}
                \caption*{mDCSRN}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x6/ax/mdsr.png}
                \caption*{3D MDSR}
            \end{subfigure}
            &
            % \hspace{-21pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x6/ax/msr.png}
                \caption*{3D RDN}
            \end{subfigure}
            &
            % \hspace{-10pt}
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x6/ax/saint.png}
                \caption*{SAINT}
            \end{subfigure}\\
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{1pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x6/sag/hr_big.png}
                \caption*{Ground Truth}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.07\linewidth}
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=2\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x6/sag/hr.png}
                \caption*{HR}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x6/sag/bicu.png}
                \caption*{Bicubic}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x6/sag/mdcsrn.png}
                \caption*{mDCSRN}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x6/sag/mdsr.png}
                \caption*{3D MDSR}
            \end{subfigure}
            &
            % \hspace{-21pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x6/sag/msr.png}
                \caption*{3D RDN}
            \end{subfigure}
            &
            % \hspace{-10pt}
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_137/x6/sag/saint.png}
                \caption*{SAINT}
            \end{subfigure}\\            
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{1pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x6/ax/hr_big.png}
                \caption*{Ground Truth}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.07\linewidth}
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=2\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x6/ax/hr.png}
                \caption*{HR}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x6/ax/bicu.png}
                \caption*{Bicubic}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x6/ax/mdcsrn.png}
                \caption*{mDCSRN}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x6/ax/mdsr.png}
                \caption*{3D MDSR}
            \end{subfigure}
            &
            % \hspace{-21pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x6/ax/msr.png}
                \caption*{3D RDN}
            \end{subfigure}
            &
            % \hspace{-10pt}
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x6/ax/saint.png}
                \caption*{SAINT}
            \end{subfigure}\\
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{1pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x6/sag/hr_big.png}
                \caption*{Ground Truth}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.07\linewidth}
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=2\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x6/sag/hr.png}
                \caption*{HR}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x6/sag/bicu.png}
                \caption*{Bicubic}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x6/sag/mdcsrn.png}
                \caption*{mDCSRN}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x6/sag/mdsr.png}
                \caption*{3D MDSR}
            \end{subfigure}
            &
            % \hspace{-21pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x6/sag/msr.png}
                \caption*{3D RDN}
            \end{subfigure}
            &
            % \hspace{-10pt}
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_176/x6/sag/saint.png}
                \caption*{SAINT}
            \end{subfigure}\\        
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{1pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x6/ax/hr_big.png}
                \caption*{Ground Truth}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.07\linewidth}
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=2\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x6/ax/hr.png}
                \caption*{HR}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x6/ax/bicu.png}
                \caption*{Bicubic}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x6/ax/mdcsrn.png}
                \caption*{mDCSRN}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x6/ax/mdsr.png}
                \caption*{3D MDSR}
            \end{subfigure}
            &
            % \hspace{-21pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x6/ax/msr.png}
                \caption*{3D RDN}
            \end{subfigure}
            &
            % \hspace{-10pt}
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x6/ax/saint.png}
                \caption*{SAINT}
            \end{subfigure}\\
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{1pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x6/sag/hr_big.png}
                \caption*{Ground Truth}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.07\linewidth}
                \setlength{\abovecaptionskip}{3pt}
                \includegraphics[width=\linewidth,height=2\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x6/sag/hr.png}
                \caption*{HR}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x6/sag/bicu.png}
                \caption*{Bicubic}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x6/sag/mdcsrn.png}
                \caption*{mDCSRN}
            \end{subfigure}
            &
            % \hspace{-2pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x6/sag/mdsr.png}
                \caption*{3D MDSR}
            \end{subfigure}
            &
            % \hspace{-21pt}
            \begin{subfigure}[b]{0.14\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x6/sag/msr.png}
                \caption*{3D RDN}
            \end{subfigure}
            &
            % \hspace{-10pt}
            \begin{subfigure}[b]{0.15\linewidth}
                \setlength{\abovecaptionskip}{2.5pt}
                \includegraphics[width=\linewidth,height=0.94\textwidth,cframe=red]{visualization_imgs/supplemental/liver_199/x6/sag/saint.png}
                \caption*{SAINT}
            \end{subfigure}\\                    
        \end{tabular}
    \caption{Visual comparisons of different methods against SAINT for $r_z = 6$. The difference maps are provided to the right of the results for better visualization.
    Images are best viewed when magnified.} \label{fig:supp_visual_x6}
    %(a) is an slice from the Kidney dataset. Despite lower PSNR value compare to RDN, SAINT generates much clearer details. (b) is a slice from the Hepatic Vessels dataset. Note that the mDCSRN result has some minor artifact due to stitching individually infered 3D cubes together
    \vspace{-1em}
\end{figure*}

==> meta.tex <==
% Current Issues in Introduction
% -- The transition to 3D SISR is too fast. What is '3D SISR' actually ? Is there any work about '3D SISR'? If not, 3D SISR is a vague term.
% -- The limitation of 3D approach is not well-presented. What does the 'zero-padding' during inference time mean?


\section{******Under Construction******}
% Two main points to justify in this paragraph. 
% - meta learning 
% - 2D approach
%
% which one goes first? 
......In this work, we aim to find a scalable approach to 3D slice interpolation for arbitrary integer sampling factors.

Recent advances in deep learning have shown promising results in solving problems such as 2D single image super-resolution (SISR) and 3D video frame interpolation [super slomo]. 

%However, existing methods cannot be directly applied for 3D slice interpolation for two main reasons. First, most existing methods only consider interpolation with a pre-determined integer scale factor. Second, there is no strong point-wise correspondence, e.g. optical flow, between consecutive slices in volumetric data

However, most existing methods only consider interpolation with a pre-determined integer scale factor. 
Recently, Hu et al. [meta-sr] proposed Meta-SR, which enables 2D SISR with arbitrary scaling factor through a meta learning upscaling module. Meta-SR dynamically predicts convolution kernels at each pixel location by taking scale- and coordinate-related vectors as input. One major drawback of this approach is its high memory consumption, which limits the image size that a network can be trained on\footnote{In [], the network is trained on patches with size 50 x 50.}. This problem becomes more prominent when we consider volumetric medical images. (Describe stitching artifact here.)  

% 3D to 2D approach & meta learning
To address these problems, we propose a new framework which is more scalable and effective than other 3D CNN alternatives. The proposed framework interpolates CT slices along the axial direction by performing a sequence of 2D SISR along sagittal and coronal directions followed by two-view fusion. The key component of the proposed framework is a novel anisotropic meta interpolation (AMI) module. Instead of predicting convolution kernels at each pixel location as in Meta-SR, AMI predicts kernels for each output channel and then applies the pixel-shuffling operation [pixel-shuffle] to achieve interpolation for arbitrary integer scale.

